OwlEyes-Online: A Fully Automated Platform for Detecting and Localizing UI Display Issues

Graphical User Interface (GUI) provides visual bridges between software apps and end users. However, due to the compatibility of software or hardware, UI display issues such as text overlap, blurred screen, image missing always occur during GUI rendering on different devices. Because these UI display issues can be found directly by human eyes, in this paper, we implement an online UI display issue detection tool OwlEyes-Online, which provides a simple and easy-to-use platform for users to realize the automatic detection and localization of UI display issues. The OwlEyes-Online can automatically run the app and get its screenshots and XML files, and then detect the existence of issues by analyzing the screenshots. In addition, OwlEyes-Online can also find the detailed area of the issue in the given screenshots to further remind developers. Finally, OwlEyes-Online will automatically generate test reports with UI display issues detected in app screenshots and send them to users. The OwlEyes-Online was evaluated and proved to be able to accurately detect UI display issues. Tool Link: http://www.owleyes.online:7476 Github Link: https://github.com/franklinbill/owleyes Demo Video Link: https://youtu.be/002nHZBxtCY

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> OwlEye_FSE_Tool (end) (Copy)(4)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> OwlEye_FSE_Tool (end) (Copy)(4)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> OwlEye_FSE_Tool (end) (Copy)(4)/figure/Illustration.tex <==
\begin{figure*}[htb]
% \vspace{0.05in}
\centering
\includegraphics[width=17cm]{figure/Illustration.png}
\vspace{-0.05in}
\caption{Illustration of our {\tool} web application.}
\label{fig:Illustration}
\vspace{-0.1in}
\end{figure*}


==> OwlEye_FSE_Tool (end) (Copy)(4)/figure/display_issues.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=8.4cm]{figure/display issues.png}
\vspace{-0.1in}
\caption{Examples of UI display issues}
\label{fig:display issues}
\vspace{-0.15in}
\end{figure}


==> OwlEye_FSE_Tool (end) (Copy)(4)/figure/overview.tex <==
\begin{figure*}[htb]
\vspace{-0.05in}
\centering
\includegraphics[width=16.5cm]{figure/overview.png}
\vspace{-0.05in}
\caption{Overview of {\tool}}
\label{fig:overview}
\vspace{-0.1in}
\end{figure*}


==> OwlEye_FSE_Tool (end) (Copy)(4)/figure/usefulness.tex <==
\begin{figure}[htb]
\centering
% \vspace{-0.1in}
\includegraphics[width=7.3cm]{figure/usefulness.png}
\vspace{-0.1in}
\caption{Average score of SUS results}
\label{fig:usefulness}
\vspace{-0.15in}
\end{figure}


==> OwlEye_FSE_Tool (end) (Copy)(4)/macro.tex <==
\usepackage{soul}
\usepackage{multirow}
\usepackage{epstopdf}
\usepackage{hyperref}
\usepackage{listings}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{ragged2e}
\usepackage{enumitem}
\usepackage[normalem]{ulem}
%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage{cleveref}

%\captionsetup[subfigure]{labelformat=simple}
%\renewcommand\thesubfigure{(\alph{subfigure})}
%\usepackage{fancybox,framed}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{tcolorbox}% http://ctan.org/pkg/tcolorbox
%\definecolor{mycolor}{rgb}{0, 0., 0}% Rule colour
\makeatletter
\newcommand{\mybox}[1]{%
  \setbox0=\hbox{#1}%
  \setlength{\@tempdima}{\dimexpr\wd0+13pt}%
  \begin{tcolorbox}[boxrule=0.5pt, colback=white, arc=4pt,
      left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt]
    #1
  \end{tcolorbox}
}
\usepackage{tikz}
\usepackage{pgfplots}
%\usepackage[usenames,dvipsnames]{xcolor}
\usetikzlibrary{pgfplots.statistics,calc}
% \usepackage{multicols}
\usepackage{color}
\usepackage{xcolor}
\usepackage{array}
\usepackage{amsmath}
\let\Bbbk\relax         %%redefined in newtxmath.sty
\usepackage{centernot}
\usepackage{xspace}
\usepackage{url}
\usepackage{verbatim}
\usepackage{wrapfig}
\usepackage{tabularx}
\clubpenalty=100000000 %10000
\widowpenalty=10000000 %10000
\brokenpenalty=10000000 %10000

\usepackage{bbding}
\usepackage{pifont}
\usepackage{wasysym}
\usepackage{amssymb}

% \newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}
% % todo commands:
% \newcommand{\todored}[1]{\todoc{red}{\textbf{[[#1]]}}}
% \newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
% \newcommand{\todoblue}[1]{\todoc{blue}{\textbf{[[#1]]}}}
% \newcommand{\todogray}[1]{\todoc{gray}{\textbf{[[#1]]}}}
% \newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
% \newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
% \newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}
%

% \newcommand{\tool}{\texttt{OwlEyes-Online}}
\newcommand{\tool}{\texttt{OwlEyes-Online}}
\newcommand{\CNN}{\texttt{CNN}}
\newcommand{\datatool}{\texttt{Data Segmentation Tool}}
\newcommand{\company}{Baidu}
\newcommand{\task}{636}

% \newcommand{\todo}[1]{\todored{TODO: #1}}
% \newcommand{\zhe}[1]{\todored{Zhe: #1}}
% \newcommand{\liuzhe}[1]{\todored{Zhe: #1}}
% \newcommand{\junjie}[1]{\todoorange{Junjie: #1}}
% \newcommand{\syhnote}[1]{\todopurple{Su: #1}}
% \newcommand{\jie}[1]{\textcolor{orange}{#1}}
% \newcommand{\add}[1]{\todoblue{#1}}
% \newcommand{\rev}[1]{\todopurple{\st{#1}}}
% \newcommand{\chen}[1]{\textcolor{red}{#1}}

%% space in some tables.  BUT have it here, such that you can always renew it
\newcommand{\ts}{$\;$}
\newcommand{\tS}{$\;$}
\newcommand{\tts}{\ \ \ \ \ }
\newcommand{\tss}{\ \ \ $\;$}
\newcommand{\ttts}{$\;$}
\newcommand{\decentHLine}{\noalign{\hrule height 1.04pt}}

%\usepackage{algorithm}  
%\usepackage{algorithmicx}  
%\usepackage{algpseudocode}


\makeatletter  
\newif\if@restonecol  
\makeatother  
%\let\algorithm\relax  
%\let\endalgorithm\relax  
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}%[ruled,vlined]{  
\usepackage{algpseudocode}  
\usepackage{amsmath}  
\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm  
\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm   

==> OwlEye_FSE_Tool (end) (Copy)(4)/sec/approach.tex <==
\section{Our Fully Automated Approach}
\label{sec_approach}
According to the features of UI display issues, we propose a fully automated UI display issue detection and localization approach. It mainly includes four parts, which are heuristic-based data generation, CNN-based issues detection, Grad CAM-based issues localization, and online inference of GUI issues.
As shown in Figure \ref{fig:overview}, to improve the accuracy of our model, we use the heuristic-based data generation method to generate a number of training data. Given an APK, {\tool} automatically runs it and collects screenshots. Then the CNN-based model classifies if they relate to any issues via the visual understanding. Once an issue is confirmed, our model can further localize its specific issue position on the UI screenshot by Grad CAM-based model to remind the developers. 

\input{figure/Illustration}

\subsection{Heuristic-based Data Generation}
\label{subsec_approach_generation}
Training our proposed CNN for issues detection requires an abundance of screenshots~\cite{ResNet} with UI display issues.
However, there is so far no such type of open dataset, and collecting the related buggy screenshots is time- and effort-consuming.
Therefore, we develop a heuristic-based data generation method for generating UI screenshots with display issues from bug-free UI images in Figure \ref{fig:overview}(a).
The data generation is based on the Rico~\cite{Rico} dataset, which contains more than 66K unique screenshots and their JSON files (i.e., detailed run-time view hierarchy of the screenshot).
With the input screenshot and its associated JSON file, we first localize all the TextView and ImageView, then randomly chooses a TextView/ImageView depending on the augmented category.
Based on the coordinates and size of the TextView/ImageView, the algorithm then makes its copy and adjusts its location or size according to specific rules to generate the screenshots with corresponding UI display issues. 

\raggedbottom

\subsection{CNN-based Issues Detection}
\label{subsec_approach_CNN}
As the UI display issues can only be spotted via the visual information, we adopt the convolutional neural network (CNN)~\cite{lecun1998gradient,krizhevsky2012imagenet}, which has proven to be effective in image classification and recognition in computer vision~\cite{VGGNet,GoogleNet,ResNet}.
Figure \ref{fig:overview}(b) shows the structure of our model, which links the convolutional layers, batch normalization layers, pooling layers, and fully connected layers.
Given the input screenshot, we convert it into a certain image size with fixed width and height as the convolutional layer's parameters consist of a set of learnable filters. 
% \syhnote{Not sure about the relation between the fixed image size with convolutional layer's parameters.}
After the convolutional layers, the screenshots will be abstracted as a feature graph. 
In order to improve the performance and stability of CNN, we add Batch Normalization (BN)~\cite{BN} layers after the convolutional layer and standardize the input layer by adjusting and scaling activation. 
After the BN layer, we add the Rectified Linear Unit (ReLU) as the activation function of the network. 
% In CNN's pooling layers, we divide feature maps into rectangular sub-regions, and the features in each rectangle are independently down-sampled to a single value.
The last several layers are fully connected neural networks (FC) which compile the data extracted by previous layers to form the final output. 
Finally, we obtain the detection results through softmax~\cite{PatternRecognition&ML}.

\raggedbottom

\subsection{Grad CAM-based Issues Localization}
\label{subsec_approach_localization}
As shown in Figure \ref{fig:overview}(c), we adopt the feature visualization method to localize the detailed position of the issues to remind the developers.
We apply the Grad-CAM model for the localization of UI display issues.
Gradient weighted Class Activation Mapping (Grad-CAM) is a technique for visualizing the regions of input that are ``important'' for predictions on CNN-based models~\cite{Grad-CAM} .
% The final convolutional layer of CNN model contains the spatial and semantic information, and this technique uses the class-specific gradient information flowing into the final convolutional layer to produce a localization map of the important regions in the inputted image. 
First, a screenshot with the UI display issue is input into the trained CNN model, and the category supervisor to which the image belongs is set to 1, while the rest is 0. 
Then the information is propagated back to the convolutional feature map of interest to obtain the Grad-CAM positioning. 
Through the feedback of global average pooling of the gradient, the weight $ \alpha_k^b $ of the importance of neurons is obtained. This weight captures the importance of the feature map $K$ of the target category $ b $ (Bug). By performing the weighted combination of the forward activation graph, we can obtain the class-discriminative localization map.
Finally, the point multiplication with the backpropagation can obtain the Grad-CAM as the result of issue localization. 

\subsection{Online Inference of GUI Issues}
\label{subsec_approach_Collection}

We use 20,000 screenshots generated in section \ref{subsec_approach_generation} to train our issue detection and localization model. Before the issue detection, we need to preprocess the APK submitted by the user online.
As shown in Figure \ref{fig:overview}(d), the user provides an Android APK, and we use the dynamic analysis method to run the app automatically to obtain the screenshots.
In detail, by leveraging the idea of dynamic app GUI testing~\cite{li2017droidbot,cai2020fastbot,Monkey,su2017guided}, we adopt an app explorer~\cite{li2017droidbot} to automatically explore the pages within an application through interacting with apps using random actions, e.g., clicking, scrolling, and filling in text. 
We also provide three testing strategies for users to choose from: Depth-First-Search (DFS)~\cite{shwail2013probabilistic}, Breadth-First-Search (BFS)~\cite{beamer2012direction}, and random exploration~\cite{Monkey}.


==> OwlEye_FSE_Tool (end) (Copy)(4)/sec/conclusion.tex <==
\section{Conclusion}
\label{sec_conclusion}

Improving the quality of mobile applications, especially in a proactive way, is of great value and always encouraged. 
In this demo, we show {\tool}, a fully automated UI display issue detection and localization tool. We use dynamic analysis to explore the application automatically and get its screenshots. And users can customize the exploration time, exploration strategy and so on. Then we can complete the detection and localization of UI display issues based on CNN and Grad-CAM. Finally, we automatically generate test reports and send them to users. 
We evaluate it from two aspects of detection accuracy and tool practicability.
The {\tool} is proven to be effective in real-world practice, i.e., 64 confirmed or fixed previously undetected UI display issues from popular Android apps.
It also achieves boosts of more than 17\% and 23\% in recall and precision compared with the best baseline.
%The proposal includes a boost of more than 21% for the EPA, 一个例句
The evaluation shows that {\tool} is a good starting point for UI display issue detection.

In the future, we will further study the root cause of UI display issue.
% combine it with program analysis technology to complete the positioning of the issue code. 
Finally, according to the issue category, we will devise a set of tools for recommending patches to developers to fix the UI display issues.

%\rev{This paper investigates a novel software linting problem - lint GUI animations against design-don't guidelines.We innovatively solve the problem using multi-class GUI animation classification.In absence of sufficient labeled data for training the classifier, we design a novel adversarial autoencoder for unsupervised representation learning of GUI animations.From a large amount of unlabeled GUI animations that are automatically collected from real applications, our model learns to extract abstract temporal-spatial feature representations from GUI animations with different fine-grained GUI content and visual effects, based on which a simple k-nearest neighbor search can accurately ``see'' the anomaly of an unseen GUI animations against a small number of (5-15) GUI animation examples of design-don't guidelines for a wide range of animation effects, screen positions and GUI components.As the first work of its kind, we also contribute two labeled and one unlabeled datasets for future research, and unveil the challenges that deserve further research in this novel software linting problem.}





==> OwlEye_FSE_Tool (end) (Copy)(4)/sec/evaluation.tex <==
\section{Evaluation}
\label{sec_evaluation}
The goal of our study is to evaluate the usefulness of our platform {\tool} in terms of (i) its effectiveness in detecting and localizing UI display issues, and (ii) the usability of our {\tool}.

\subsection{Effectiveness Measurement}
\label{sec_effectiveness}

Given the effectiveness of our {\tool} for UI display issue detection, we conduct experiments on 8K Android mobile GUI collected by one of the largest crowd-testing platforms~\cite{BaiduC}.
% \footnote{Baidu (baidu.com) is the largest Chinese search service provider.
% Its crowdsourcing test platform (test.baidu.com) is also one of the
% largest in China.}. 
This part is also published in our previous work~\cite{liu2020owl} and and we mainly use evaluation metrics of precision and recall.

Table \ref{tab:RQ2-Baseline} shows the performance comparison with the baselines. 
With {\tool}, the precision is 0.85 and the recall is 0.84.
We can see that our proposed {\tool} is much better than the baselines, i.e., 58\% higher in precision and 17\% higher in recall compared with the best baseline, Multilayer Perceptron (MLP).
This further indicates the effectiveness of {\tool}.
Besides, it also implies that {\tool} is especially good at hunting for the buggy screenshots from candidate ones, i.e., significant improvement in recall.

\input{tab/baseline1.tex}

% We further analyze the screenshots which are wrongly predicted as bug-free.
% One common shared by these screenshots is that the buggy area is too tiny to be recognized even with human eyes. 
% Future work will focus more on improving the detection performance for these screenshots with attention mechanism and image magnification.

\subsection{Usefulness Measurement}
\label{sec_usefulness}

To further assess the usefulness of our approach, we randomly sample 2,000 Android applications from F-Droid~\cite{F-droid} and 1,000 applications from Google Play~\cite{GooglePlay}.
Note that none of these apps appears in our training dataset.
Among the 3,000 collected applications, 59\% (1756/3000) applications can be successfully run with {\tool}.
For the remaining 1,756 applications, an average of 8 screenshots is obtained for each application. 
We then feed those screenshots to our {\tool} and detect if there are any display issues.
Once a display issue is spotted, we create a bug report by describing the issue attached with a buggy UI screenshot.
Finally, we report them to the app development team through issue reports or emails. 
Our {\tool} has detected 113 UI display issues, among which 35 have been confirmed and 29 have been fixed.
These fixed or confirmed bug reports further demonstrate the effectiveness and usefulness of our proposed approach in detecting UI display issues. 

Regarding the user experience of our {\tool}, we create an online survey on 20 professional developers, testers, and researchers, all of whom major in computer science with more than 3 years of app testing or developing experience. 10 of them are from the industry with practical working experience\footnote{Some testers are from NVIDIA, Citibank, Sony, Baidu, Alibaba, Three Fast Online, and ByteDance.}. We ask them to use our {\tool} and ask them about the usefulness of the {\tool} for their work, as well as its potential and scalability in the future. In the end, participants fill in the System Usability Scale (SUS) questionnaire~\cite{brooke1996sus} (5-point Likert scale~\cite{5-likert-1} from 1 (strongly disagree) to 5 (strongly agree)). The questionnaire also asks participants to select the TechLand system features that they deem most useful or least useful for the tasks.

\input{figure/usefulness}

Figure \ref{fig:usefulness} summarizes the participants’ ratings of the 10 system design and usability questions in the System Usability Scale questionnaire. The upper half of figure \ref{fig:usefulness} shows that participants agree or strongly agree that our system is easy to use and the features of the {\tool} system are well-devised. The lower half of figure \ref{fig:usefulness} further confirms the simplicity and consistency of our {\tool} system. Furthermore, the average helpfulness of the {\tool} system for the tasks is 4.42, which indicates that participants appreciate the help of the {\tool} system in the tasks.
All participants indicated that {\tool} has a good UI display issue detection effect. Among these professionals, 10 of them are working on app testing. They think {\tool} can help them localize the UI display issues more quickly. 7 Android developers said that our issue localization model helps them better localize the issue on the UI interface so that they can better repair the issue later. Among them, 4 developers hope we can further give the possible repair methods and causes of these issues. The other 3 participants who are studying GUI testing also indicated that they hope we can analyze the cause of issue in the next stage. They think that using the visual information of application screenshots is a very helpful and engaging work.

==> OwlEye_FSE_Tool (end) (Copy)(4)/sec/implementation.tex <==
\section{Tool Implementation And Usage}
\label{sec_implementation}

{\tool} is a web app, which provides a convenient tool for users to detect and localize the UI display issues in the GUI screenshots.

\subsection{Web Implementation}
\label{subsec_Web}
{\tool} can automatically run applications and generate test reports for users. We customized the deep learning model in PyTorch. The {\tool} consists of two parts: running the application automatically, feeding back the test results in real-time.

\textbf{Running the app automatically:} Figure \ref{fig:Illustration}(a) shows an example of our running the app automatically page. Users can upload the APK or its download link. In addition, we allow users to customize the exploration strategy, select the appropriate device, and some personalization settings to provide a more friendly interactive experience.

\textbf{The Real-time feedback issue detection results:} This page in Figure \ref{fig:Illustration}(b) will give real-time feedback test results while running the application automatically. On this page, we implement some functions to provide a more friendly interactive experience, including:

\textbf{Click to view the localization details:} In Figure \ref{fig:Illustration}(c), click the screenshot of the UI display issue to view the localization of it in the screenshot (in the form of a thermal graph).

\textbf{Export test report}: In Figure \ref{fig:Illustration}(d), users fill in e-mail information, and we will automatically generate test reports and send them to users. The test report includes the number of issues of the application and the screenshots of the issue and the XML corresponding to the screenshots.

\raggedbottom


\subsection{Model Implementation}
\label{subsec_Model}
Our CNN model is composed of 12 convolutional layers with batch normalization, 6 pooling layers, and 4 full connection layers for classifying UI screenshot with display issues. 
The size of a convolutional kernel in the convolutional layer is 3 $\times$ 3. We set up the number of convolutional kernels as 16 for convolutional layer 1-4, 32 for convolutional layer 5-6, 64 for convolutional layer 7-8, and 128 for convolutional layer 9-12. 
For the pooling layers, we use the most common-used max-pooling settings~\cite{simard2003best}, i.e., pooling units of size 2 $\times$ 2 applied with a stride ~\cite{VGGNet}. 
We set the number of neurons in each of the fully connected layers as 4096, 1024, 128, and 2 respectively.
For data preprocessing, we rotate some UI of the horizontal screens to vertical, and resize the screens to 768 $\times$ 448. 
We implement our model based on the PyTorch~\cite{pytorch} framework. 
The model is trained in an NVIDIA GeForce RTX 2060 GPU (16G memory) with 100 epochs for about 8 hours.

\subsection{Usage Scenarios}
\label{subsec_Usage}

We present several examples to illustrate how developers would interact with {\tool}. In some cases, developers collect a large number of screenshots of applications (such as crowdtesting platform, automatic testing). However, these automated tools can only spot critical crash bugs, rather than UI display issues that cannot be captured by common tools. Developers can upload application screenshots to our {\tool} directly. {\tool} will analyze the screenshots and detect the UI display issue in the screenshots.

For testing whether UI display issues exist in the application, developers can directly upload an APK to our {\tool} , which will automatically explore the application and detect UI display issues. Developers can also customize the exploration method and duration and submit the e-mail information. After the issue detection, {\tool} will automatically generate the issue report and send it to the developer's e-mail. Considering the network delay, developers can also upload an application's download link, and {\tool} will automatically download the APK in the background for testing.

==> OwlEye_FSE_Tool (end) (Copy)(4)/sec/introduction.tex <==
\section{Introduction}
\label{sec_introduction}
GUI is widely used among modern mobile apps, making it practical and easy to use.
However, with the development of visual effects of GUI, five categories of UI display issues~\cite{liu2020owl} such as \textit{component occlusion, text overlap, missing image, null value} and \textit{blurred screen} always occur during the UI display process, especially on different mobile devices.
Detecting those issues is a hard problem because most of those UI display issues are caused by many factors, especially for Android, such as different Android OS versions, device models, and screen resolutions~\cite{wei2016taming}. 
% To gather those issues, the common measure is to recruit testers for application GUI testing or leverage crowdtesting, which requires significant human efforts to test apps.
Nowadays, some practical automated testing tools like Monkey~\cite{Monkey, Wetzlmaier2017Hybrid}, Dynodroid~\cite{Dynodroid} are also widely used in industry.
However, these automated tools can only spot critical crash bugs, rather than UI display issues that cannot be captured by common tools. Inspired by the fact that display bugs can be easily spotted by human eyes, we develop an automated online tool {\tool}\footnote{{\tool} is named as our approach is like the owl's eyes to effectively spot UI display issues. And our model (nocturnal like an owl) can complement conventional automated GUI testing (diurnal like an eagle) for ensuring the robustness of the UI.}, which provides quick detection and localization of UI display issues from apps or GUI screenshots.

\input{figure/overview.tex}

The {\tool} is a user-friendly web app. Developers can upload GUI screenshots or apps and receive accurate UI display issue detection results. When a developer uploads an APK, it will automatically run the app and get its screenshots, and then we use computer vision technologies to detect the UI display issues.
{\tool} builds on the CNN to identify the screenshots with issues and Grad-CAM to localize the regions with UI display issues in the screenshots for further reminding developers. 
Finally, it summarizes the detection and localization results, automatically generates the test report and sends it to users.
Considering that the CNN needs lots of training data, we adopt a heuristic data generation method to generate the training data.

% The {\tool} is a user-friendly web app. Developers can upload GUI screenshots or apps and receive accurate UI display issue detection results. When a developer uploads an APK, {\tool} will automatically run the app and get its screenshots, and then we use computer vision technologies to detect the UI display issues.
% {\tool} builds on the CNN to identify the screenshots with issues and Grad-CAM to localize the regions with UI display issues in the screenshots for further reminding developers. 
% Finally, the {\tool} summarizes the detection and localization results, automatically generates the test report and sends it to users.
% Considering that the CNN needs lots of training data, and the element UI style of the updated app version will change, we adopt a heuristic data generation method to generate a large number of training data from the bug-free screenshots.
% , so as to improve the detection accuracy and robustness of {\tool}.

{\tool} provides a dashboard for users to upload the screenshots or apps.
% , where users can pick up a preferred app to analyze and customize the exploration time or choose a UI screenshot to analyze. 
After analyzing an uploaded screenshot, it displays detection results in real-time. As for an app, it automatically generates a test report (issue screenshots, localization, etc.) and sends the report to the user in an email.

This paper makes the following contributions:
\begin{itemize}
\item We implement a CNN based issue detection method and a Grad-CAM based issue localization method to detect UI display issues from GUI screenshots.

\item We develop a fully automated web app. Users only need to upload an APK file, and {\tool} will automatically generate test reports and send them to users. We release the implementation of {\tool} on Github~\cite{GithubLink}.

\item An empirical study among professionals proves the value of our UI display issue detection method and {\tool}.

\end{itemize}


==> OwlEye_FSE_Tool (end) (Copy)(4)/tab/baseline1.tex <==
\begin{table}[H]
\vspace{-0.1in}
\caption{Performance comparison with baselines}
\vspace{-0.1in}
\label{tab:RQ2-Baseline}
\centering
\footnotesize
\begin{tabular}{p{1.7cm}<{\centering} | p{1.5cm}<{\centering} | p{1.5cm}<{\centering} | p{1.5cm}<{\centering}}
\hline
\textbf{Method} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
%\hline
%\multicolumn{4}{c}{\textbf{SIFT Feature Detection Algorithm}} \\
\hline
% SIFT-SVM & 0.486 & 0.349 & 0.406 \\ 
% %\hline
% SIFT-KNN & 0.510 & 0.492 & 0.501 \\ 
% %\hline
% SIFT-NB & 0.584 & 0.411 & 0.482 \\ 
% %\hline
RF-SIFT & 0.458 & 0.458 & 0.432 \\ 
%\hline
%\multicolumn{4}{c}{\textbf{SURF Feature Detection Algorithm}} \\
% \hline
% SURF-SVM & 0.561 & 0.512 & 0.535 \\ 
% %\hline
% SURF-KNN & 0.522 & 0.526 & 0.524 \\ 
% %\hline
% SURF-NB & 0.428 & 0.597 & 0.499 \\ 
% %\hline
RF-SURF & 0.513 & 0.524 & 0.519 \\ 
%\hline
%\multicolumn{4}{c}{\textbf{ORB Feature Detection Algorithm}} \\
% \hline
% ORB-SVM & 0.551 & 0.514 & 0.532 \\ 
% %\hline
% ORB-KNN & 0.525 & 0.522 & 0.523 \\ 
% %\hline
% ORB-NB & 0.567 & 0.709 & 0.630 \\ 
%\hline
RF-ORB & 0.520 & 0.528 & 0.524 \\  
%\hline
%\multicolumn{4}{c}{\textbf{Deep Learning}} \\
\hline
MLP & 0.537 & 0.727 & 0.618 \\  
%\hline
%\multicolumn{4}{c}{\textbf{Our method}} \\
\hline
\textbf{{\tool}} & \textbf{0.850} & \textbf{0.848} & \textbf{0.849} \\ 
\hline
\end{tabular}
\vspace{-0.1in}
\end{table}


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> figure/display_issues.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=8.4cm]{figure/display issues.png}
\vspace{-0.1in}
\caption{Examples of UI display issues}
\label{fig:display issues}
\vspace{-0.15in}
\end{figure}


==> macro.tex <==
\usepackage{soul}
\usepackage{multirow}
\usepackage{epstopdf}
\usepackage{hyperref}
\usepackage{listings}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{ragged2e}
\usepackage{enumitem}
\usepackage[normalem]{ulem}
%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage{cleveref}

%\captionsetup[subfigure]{labelformat=simple}
%\renewcommand\thesubfigure{(\alph{subfigure})}
%\usepackage{fancybox,framed}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{tcolorbox}% http://ctan.org/pkg/tcolorbox
%\definecolor{mycolor}{rgb}{0, 0., 0}% Rule colour
\makeatletter
\newcommand{\mybox}[1]{%
  \setbox0=\hbox{#1}%
  \setlength{\@tempdima}{\dimexpr\wd0+13pt}%
  \begin{tcolorbox}[boxrule=0.5pt, colback=white, arc=4pt,
      left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt]
    #1
  \end{tcolorbox}
}
\usepackage{tikz}
\usepackage{pgfplots}
%\usepackage[usenames,dvipsnames]{xcolor}
\usetikzlibrary{pgfplots.statistics,calc}
% \usepackage{multicols}
\usepackage{color}
\usepackage{xcolor}
\usepackage{array}
\usepackage{amsmath}
\let\Bbbk\relax         %%redefined in newtxmath.sty
\usepackage{centernot}
\usepackage{xspace}
\usepackage{url}
\usepackage{verbatim}
\usepackage{wrapfig}
\usepackage{tabularx}
\clubpenalty=100000000 %10000
\widowpenalty=10000000 %10000
\brokenpenalty=10000000 %10000

\usepackage{bbding}
\usepackage{pifont}
\usepackage{wasysym}
\usepackage{amssymb}

% \newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}
% % todo commands:
% \newcommand{\todored}[1]{\todoc{red}{\textbf{[[#1]]}}}
% \newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
% \newcommand{\todoblue}[1]{\todoc{blue}{\textbf{[[#1]]}}}
% \newcommand{\todogray}[1]{\todoc{gray}{\textbf{[[#1]]}}}
% \newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
% \newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
% \newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}
%

% \newcommand{\tool}{\texttt{OwlEyes-Online}}
\newcommand{\tool}{\texttt{OwlEyes-Online}}
\newcommand{\CNN}{\texttt{CNN}}
\newcommand{\datatool}{\texttt{Data Segmentation Tool}}
\newcommand{\company}{Baidu}
\newcommand{\task}{636}

% \newcommand{\todo}[1]{\todored{TODO: #1}}
% \newcommand{\zhe}[1]{\todored{Zhe: #1}}
% \newcommand{\liuzhe}[1]{\todored{Zhe: #1}}
% \newcommand{\junjie}[1]{\todoorange{Junjie: #1}}
% \newcommand{\syhnote}[1]{\todopurple{Su: #1}}
% \newcommand{\jie}[1]{\textcolor{orange}{#1}}
% \newcommand{\add}[1]{\todoblue{#1}}
% \newcommand{\rev}[1]{\todopurple{\st{#1}}}
% \newcommand{\chen}[1]{\textcolor{red}{#1}}

%% space in some tables.  BUT have it here, such that you can always renew it
\newcommand{\ts}{$\;$}
\newcommand{\tS}{$\;$}
\newcommand{\tts}{\ \ \ \ \ }
\newcommand{\tss}{\ \ \ $\;$}
\newcommand{\ttts}{$\;$}
\newcommand{\decentHLine}{\noalign{\hrule height 1.04pt}}

%\usepackage{algorithm}  
%\usepackage{algorithmicx}  
%\usepackage{algpseudocode}


\makeatletter  
\newif\if@restonecol  
\makeatother  
%\let\algorithm\relax  
%\let\endalgorithm\relax  
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}%[ruled,vlined]{  
\usepackage{algpseudocode}  
\usepackage{amsmath}  
\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm  
\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm   
